BOOSTEDSOSA: Accelerated Inferencing for Low Variance Stochastic Online Scheduling

Heterogeneous scheduling in stochastic, online envi- ronments, such as high-performance computing (HPC) systems, presents a significant challenge. Stochastic Online Scheduling Accelerators (SOSAs) offer a promising solution, but their effectiveness is compromised by a reliance on runtime estimates provided by users. These estimates introduce substantial vari- ance into the scheduling process (mean MAE in hundreds of Core-Days), thereby weakening the competitiveness of Stochastic Online Scheduling algorithms as their competitive-ratio bound increases with runtime variability. To address this limitation, we introduce BOOSTEDSOSA, a dual-FPGA ML-assisted Scheduling architecture that integrates a Machine Learning predictor for expected processing times, with a novel temporal-aware training policy. The predictor estimates job runtimes using only scheduler parameters available at submission time, enabling its use in existing HPC systems. Using historical real-world HPC job data (from the Argonne Leadership Comput- ing Facility, MIT Supercloud and UIUC Blue Waters workload datasets), we show that the predictor reduces MAE by up to 63.85% compared to user runtime estimates, and the additive training policy reduces MAE by up to 71.88% compared to a static model. End-to-end, BOOSTEDSOSA achieves an average 17x speedup over an AVX-optimized software baseline and processes up to 1,711 jobs/seconds

==> tables/XGB_vs_RF.tex <==
\begin{table}[htpb]
\centering
\small
\caption{MAE across 5-fold cross-validation. ADD (XGB) consistently achieves the lowest error across every individual fold and the overall mean.}
\label{tab:XGB_RF_table}
\begin{tabular}{lccc}
\toprule
\textbf{Fold} & \textbf{CORE (Agg)} & \textbf{ADD (RF)} & \textbf{ADD (XGB)} \\
\midrule
1 & 1,097.4 & 970.4 & \textbf{926.8} \\
2 & 1,080.9 & 959.6 & \textbf{894.9} \\
3 & 1,085.4 & 960.3 & \textbf{912.4} \\
4 & 1,103.3 & 971.8 & \textbf{922.1} \\
5 & 1,084.9 & 963.2 & \textbf{910.8} \\
\midrule
\textbf{Mean} & 1,090.4 & 965.1 & \textbf{913.4} \\
\bottomrule
\end{tabular}
\end{table}
